Discovery of Gas Accretion Onto Stars in 13 Myr old h and chi Persei

We report the discovery of accretion disks associated with ~ 13 Myr-old intermediate/low-mass stars in h and chi Persei. Optical spectroscopy of ~ 5000 stars in these clusters and a surrounding halo population reveal 32 A-K stars with H(alpha) emission. Matching these stars with 2MASS and optical photometry yields 25 stars with the highest probability of cluster membership and EW(H(alpha)) > 5 angstroms. Sixteen of these sources have EW(H(alpha)) > 10 angstroms. The population of accreting sources is strongly spectral type dependent: H(alpha) emission characteristic of accretion, especially strong accretion (EW(H(alpha)) > 10 angstroms), is much more prevalent around stars later than G0. Strong H(alpha) emission from accretion is typically associated with redder Ks-[8] colors. The existence of accreting pre-main sequence stars in h and chi Persei implies that circumstellar gas in some systems, especially those with primaries later than G5 spectral type, can last longer than 10-15 Myr.

==> tab1f.tex <==
\begin{deluxetable}{lllllllllllllll}
\tiny
%\rotate
%\documentstyle[10pt]
%SPMquot"(0pt)
%\setlength{\tabcolstep}{0.02in}
%\linewidth{0.1 in}
%\tabletypesize{\tiny}
\tablewidth{0pt}
\tabletypesize{\scriptsize}
\tablecolumns{10}
\tablecaption{H$_{\alpha}$ emission sources}
\tiny
\tablehead{{$\alpha$}&{$\delta$}&{ST}&{$\sigma$(ST, subclasses)}&{EqW(H$_{\alpha}$)}&{Accreting?}&{J}&{K$_{s}$}&{K$_{s}$-[3.6]}&{K$_{s}$-[8]}}
\startdata
 2:22:21.62  &  57:04:00.5  &   G4   &    1.00   &   13.74   &   y  &   14.303   &    13.612   &     0.292  &\ldots  \\
   2:22:39.53  &  57:15:42.9  &   G0   &    2.50   &    4.50   &   n  &   14.315   &    13.538   &     0.271  &    0.223  \\
   2:17:36.96  &  57:01:10.6  &   G0   &    3.00   &    1.80   &   n  &   14.363   &    13.697   & \ldots  &   -0.247  \\
   2:17:55.15  &  56:56:03.1  &   G3   &    2.10   &    6.46   &   y  &   14.419   &    13.613   &     0.258  &    0.096  \\
   2:21:46.44  &  57:02:44.2  &   G4   &    2.30   &    5.75   &   y  &   14.446   &    13.697   &     0.349  &    0.405  \\
   2:22:04.13  &  57:22:49.5  &   F9   &    1.80   &    3.40   &   n  &   14.461   &    13.549   &     0.087  &    0.043  \\
   2:20:14.30  &  56:44:21.5  &   G1   &    2.40   &   12.40   &   y  &   14.638   &    14.042   &   \ldots  &  \ldots  \\
   2:20:52.37  &  57:13:04.8  &   G6   &    0.60   &    8.50   &   y  &   14.706   &    13.830   &     0.103  &    0.326  \\
   2:23:23.45  &  57:03:25.2  &   G0   &    2.20   &    3.20   &   n  &   14.707   &    14.038   &     0.337  &    0.221  \\
   2:18:05.71  &  57:18:58.3  &   G2   &    2.10   &   15.42   &   y  &   14.728   &    14.024   &     0.295  &    0.471  \\
   2:18:05.38  &  57:01:28.2  &  G3   &    2.20   &   10.15   &   y  &   14.779   &    13.972   &     0.041  &    0.274  \\
   2:20:36.74  &  57:05:36.6  &   G2   &    2.30   &    8.98   &   y  &   14.780   &    13.941   &     0.130  &    0.357  \\
   2:23:32.88  &  57:06:57.2  &   G5   &    2.60   &    8.60   &   y  &   14.782   &    14.065   & \ldots  &    0.342  \\
   2:17:07.32  &  57:11:12.8  &   G4   &    1.30   &    9.79   &   y  &   14.795   &    14.174   &     0.362  &\ldots  \\
   2:22:30.62  &  57:14:34.4  &   G7   &    1.20   &   12.93   &   y  &   14.852   &    14.049   &     0.143  &\ldots  \\
   2:22:48.62  &  57:12:36.7  &   G8   &    0.58   &    7.90   &   y  &   14.880   &    14.128   &     0.346  &    0.230  \\
   2:21:39.70  &  57:16:49.4  &   G5   &    2.50   &   12.74   &   y  &   14.886   &    14.028   &     0.155  &    0.183  \\
   2:22:37.78  &  57:13:04.1  &   G0   &    2.00   &    2.86   &   n  &   14.900   &    14.167   &   \ldots  &  \ldots  \\
   2:22:06.86  &  57:07:45.1  &   K1   &    1.20   &   13.07   &   y  &   14.948   &    13.988   &   \ldots  &  \ldots  \\
   2:21:32.57  &  57:00:32.0  &   G0   &    3.00   &    5.00   &   y  &   14.970   &    14.262   &     0.205  &\ldots  \\
   2:21:36.22  &  57:11:08.9  &   G2   &    2.00   &   23.00   &   y  &   15.026   &    14.290   &     0.265  &\ldots  \\
   2:21:57.91  &  57:04:04.8  &   K0   &    0.96   &   12.96   &   y  &   15.281   &    14.399   &     0.348  &    0.372  \\
   2:19:06.70  &  56:52:17.8  &   K1   &    1.50   &    8.80   &   y  &   15.321   &    14.563   &     0.311  &\ldots  \\
   2:21:35.86  &  57:05:22.9  &   K3   &    3.00   &   29.93   &   y  &   15.364   &    14.286   &     0.069  &\ldots  \\
   2:17:48.48  &  57:23:31.9  &   K2   &    1.20   &   19.40   &   y  &   15.368   &    14.411   &     0.287  &\ldots  \\
   2:18:36.46  &  57:01:15.2  &   G6   &    2.00   &   11.59   &   y  &   15.394   &    14.427   &     0.091  &    0.231  \\
   2:21:15.62  &  57:04:37.9  &   K2.5   &    1.20   &   26.40   &   y  &   15.554   &    14.401   &     0.053  &    0.328  \\
   2:17:38.69  &  57:26:46.0  &   K4   &    2.00   &   59.50   &   y  &   15.822   &    15.077   &     0.452  &\ldots  \\
   2:18:11.74  &  57:04:43.0  &   K7   &    2.50   &   47.32   &   y  &   16.552   &    14.827   & \ldots  &    0.937  \\
   2:18:39.00  &  57:10:14.2  &   A7   &    2.00   &   11.50   &   y  &   14.150   &    13.889   &     0.123  &    0.186  \\
\enddata
\tablecomments{Properties of sources with H$_{\alpha}$ emission (first five entries).
Sources with EW(H$_{\alpha}$), $\ge$ 5\AA\ are identified as accreting sources.
 All but the final entry are from Hectospec.
Uncertainties in EW(H$_{\alpha}$) were $\sim$ 1-2 \AA\.
All photometric measurements listed are 5$\sigma$ detections.
Sources were typically brighter than the 10$\sigma$ limit in
J (15.7) and K$_{s}$ (14.8) (see \citealt{Cu07a}).}
\end{deluxetable}

